Signaling Human Intentions to Service Robots: Understanding the Use of Social Cues during In-Person Conversations

As social service robots become commonplace, it is essential for them to effectively interpret human signals, such as verbal, gesture, and eye gaze, when people need to focus on their primary tasks to minimize interruptions and distractions. Toward such a socially acceptable Human-Robot Interaction, we conducted a study ($N=24$) in an AR-simulated context of a coffee chat. Participants elicited social cues to signal intentions to an anthropomorphic, zoomorphic, grounded technical, or aerial technical robot waiter when they were speakers or listeners. Our findings reveal common patterns of social cues over intentions, the effects of robot morphology on social cue position and conversational role on social cue complexity, and users' rationale in choosing social cues. We offer insights into understanding social cues concerning perceptions of robots, cognitive load, and social context. Additionally, we discuss design considerations on approaching, social cue recognition, and response strategies for future service robots.

==> sections/method/tab-codebook.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\begin{longtable}[c]{|c|c|cc|c|}
\caption{caption}
\label{tab: codebook}\\
\toprule
Modality & Code Type & \multicolumn{1}{c|}{Category} & Code & \#labels \\* \midrule
\endfirsthead
%
\multicolumn{5}{c}%
{{\bfseries Table \thetable\ continued from previous page}} \\
\toprule
Modality & Code Type & \multicolumn{1}{c|}{Category} & Code & \#labels \\* \midrule
\endhead
%
\multirow{41}{*}{Arm and Hand Gesture} & \multirow{32}{*}{Articulation Code} & \multicolumn{1}{c|}{\multirow{32}{*}{Gesture Name}} & dismissive wave & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & beckoning wave & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & wave & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & palm point to send away the robot & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & palm to stop the robot & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & palm inwards and fingers point down & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & thumb up & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & thumb down & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & hand press down & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & ok & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & number & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & shake index finger & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & palm point to robot & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & palm point across the table & 9 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & palm point to the place & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & palm point to the drink & 7 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & palm point from robot to across table & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & palm point from across table to robot & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & finger point from robot to across table & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & finger point from across table to robot & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & index finger point to the drink & 7 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & index finger point to the place & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & index finger point to partner & 9 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & index finger point to robot & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & finger point to distant & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & hold the drink & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & tap the table & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & shuuu & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & hand beside mouth & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & spread both hands & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & cross two fingers to show no & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & stop (index finger+palm) & 3 \\* \cmidrule(l){2-5} 
 & \multirow{9}{*}{Feature Code} & \multicolumn{2}{c|}{Moving Extent} & 4 \\* \cmidrule(l){3-5} 
 &  & \multicolumn{2}{c|}{Moving Speed} & 4 \\* \cmidrule(l){3-5} 
 &  & \multicolumn{2}{c|}{Repetition} & 3 \\* \cmidrule(l){3-5} 
 &  & \multicolumn{2}{c|}{Handedness} & 4 \\* \cmidrule(l){3-5} 
 &  & \multicolumn{1}{c|}{\multirow{4}{*}{Hand Position}} & hand height & 5 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & in front of face & 2 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & behind body & 2 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & hand rest on table & 2 \\* \cmidrule(l){3-5} 
 &  & \multicolumn{2}{c|}{Distance from Body} & 4 \\* \midrule
\multirow{13}{*}{Verbal} & \multirow{2.3}{*}{Articulation Code} & \multicolumn{2}{c|}{Exact Content} & 2 \\* \cmidrule(l){3-5} 
 &  & \multicolumn{2}{c|}{Speech Act} & 6 \\* \cmidrule(l){2-5} 
 & \multirow{11}{*}{Feature Code} & \multicolumn{2}{c|}{Unclear Reference} & 2 \\* \cmidrule(l){3-5} 
 &  & \multicolumn{1}{c|}{\multirow{9}{*}{Politeness}} & Apology & 2 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & Could You & 2 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & First-Person Plural & 2 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & Gratitude & 2 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & Hello & 2 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & Please & 2 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & Positive Emotion & 2 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & Reasoning & 2 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & Subjectivity & 2 \\* \cmidrule(l){3-5} 
 &  & \multicolumn{2}{c|}{Volume} & 4 \\* \midrule
\multirow{4}{*}{Eye} & \multirow{4}{*}{Articulation Code} & \multicolumn{1}{c|}{\multirow{4}{*}{Eye Gaze}} & turn to the robot & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & turn to the drink & 7 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & turn to across the table & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & turn to the place & 3 \\* \midrule
\multirow{10.5}{*}{Head} & \multirow{10.5}{*}{Articulation Code} & \multicolumn{1}{c|}{\multirow{4}{*}{Head Gaze}} & turn to robot & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & turn to drink & 7 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & turn to across the table & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & turn to the place & 3 \\* \cmidrule(l){3-5} 
 &  & \multicolumn{1}{c|}{\multirow{4}{*}{Head Movement}} & turn to the side & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & shake & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & nod & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & jaw point to across the table & 3 \\* \midrule
\multirow{3}{*}{Upper\_Body} & \multirow{3}{*}{Articulation Code} & \multicolumn{1}{c|}{\multirow{3}{*}{Body orientation relative to chair}} & lean left & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & lean right & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & lean back & 3 \\* \midrule
\multirow{4}{*}{Other\_Facial} & \multirow{4}{*}{Articulation Code} & \multicolumn{1}{c|}{\multirow{4}{*}{Facial}} & purse the lips & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & frown & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & raise eyebrow & 3 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & smile & 3 \\* \midrule
\multirow{4}{*}{Leg\_and\_Foot} & \multirow{4}{*}{Articulation Code} & \multicolumn{1}{c|}{\multirow{4}{*}{Foot}} & stamp & 2 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & foot draw circle & 2 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & foot draw line & 2 \\* \cmidrule(l){4-5} 
 &  & \multicolumn{1}{c|}{} & kick away & 2 \\* \bottomrule
\end{longtable}
